Throughput-Optimal Broadcast in Wireless Networks with Point-to-Multipoint Transmissions

We consider the problem of efficient packet dissemination in wireless networks with point-to-multi-point wireless broadcast channels. We propose a dynamic policy, which achieves the broadcast capacity of the network. This policy is obtained by first transforming the original multi-hop network into a precedence-relaxed virtual single-hop network and then finding an optimal broadcast policy for the relaxed network. The resulting policy is shown to be throughput-optimal for the original wireless network using a sample-path argument. We also prove the NP-completeness of the finite-horizon broadcast problem, which is in contrast with the polynomial time solvability of the problem with point-to-point channels. Illustrative simulation results demonstrate the efficacy of the proposed broadcast policy in achieving the full broadcast capacity with low delay.

==> extension.tex <==
\section{Extension to Networks with Noisy Channels} \label{extension}
We can extend the algorithm to the network with dynamic setting where once a packet is broadcasted by a node, it reaches each of its neighboring nodes independently with probability $p$. The parameter $p$ is assumed to be known in advance. 
\textbf{Question :} What is the capacity of the network in this setting (a lower-bound, upper-bound, exact expression)?  

==> overview.tex <==
\section{Overview of the Broadcast Policy} \label{overview}
 
